Improving UE Energy Efficiency through Network-aware Video Streaming over 5G

Adaptive Bitrate (ABR) Streaming over the cellular networks has been well studied in the literature; however, existing ABR algorithms primarily focus on improving the end-users' Quality of Experience (QoE) while ignoring the resource consumption aspect of the underlying device. Consequently, proactive attempts to download video data to maintain the user's QoE often impact the battery life of the underlying device unless the download attempts are synchronized with the network's channel condition. In this work, we develop EnDASH-5G -- a wrapper over the popular DASH-based ABR streaming algorithm, which establishes this synchronization by utilizing a network-aware video data download mechanism. EnDASH-5G utilizes a novel throughput prediction mechanism for 5G mmWave networks by upgrading the existing throughput prediction models with a transfer learning-based approach leveraging publicly available 5G datasets. It then exploits deep reinforcement learning to dynamically decide the playback buffer length and the video bitrate using the predicted throughput. This ensures that the data download attempts get synchronized with the underlying network condition, thus saving the device's battery power. From a thorough evaluation of EnDASH-5G, we observe that it achieves a near $30.5\%$ decrease in the maximum energy consumption than the state-of-the-art Pensieve ABR algorithm while performing almost at par in QoE.

==> tex/04.evaluation.tex <==
\section{Evaluation}
In this section we evaluate EnDASH and compare its perfor-
mance with other popular ABR algorithms, in terms of QoE
and energy consumption. We first discuss the methodology
that we have adopted.

	\subsection{Methodology}
	To train and test the throughput engine of EnDASH, we
	have used a corpus of throughput and power consumption
	traces collected under user mobility, for video streaming workloads. We have collected data in our ns-3 simulation environment\ref{8344116}. The baseline ABR streaming algorithms that we have used are BOLA, Pensieve, Fast MPC, and Robust MPC.
